Gaussian Processes for real-time 3D motion and uncertainty estimation during MR-guided radiotherapy

Respiratory motion during radiotherapy causes uncertainty in the tumor's location, which is typically addressed by an increased radiation area and a decreased dose. As a result, the treatments' efficacy is reduced. The recently proposed hybrid MR-linac scanner holds the promise to efficiently deal with such respiratory motion through real-time adaptive MR-guided radiotherapy (MRgRT). For MRgRT, motion-fields should be estimated from MR-data and the radiotherapy plan should be adapted in real-time according to the estimated motion-fields. All of this should be performed with a total latency of maximally 200 ms, including data acquisition and reconstruction. A measure of confidence in such estimated motion-fields is highly desirable, for instance to ensure the patient's safety in case of unexpected and undesirable motion. In this work, we propose a framework based on Gaussian Processes to infer 3D motion-fields and uncertainty maps in real-time from only three readouts of MR-data. We demonstrated an inference frame rate up to 69 Hz including data acquisition and reconstruction, thereby exploiting the limited amount of required MR-data. Additionally, we designed a rejection criterion based on the motion-field uncertainty maps to demonstrate the framework's potential for quality assurance. The framework was validated in silico and in vivo on healthy volunteer data (n=5) acquired using an MR-linac, thereby taking into account different breathing patterns and controlled bulk motion. Results indicate end-point-errors with a 75th percentile below 1mm in silico, and a correct detection of erroneous motion estimates with the rejection criterion. Altogether, the results show the potential of the framework for application in real-time MR-guided radiotherapy with an MR-linac.

==> sections/extra_.tex <==
\subsubsection{Derivation of posterior distribution of the motion-field}
Besides the posterior distribution \autoref{eq:gpposterior_general} over motion-field representation coefficients, a posterior distribution of the motion-field at time $t$ can be derived by applying the motion model $\bm{\Phi}$ to the distribution of representation coefficients. Since a linear transformation of a Gaussian distribution yields another Gaussian distribution, we can derive
\begin{equation}
    \label{eq:gp_dvf_distribution}
    \bv{D}_t := \overline{\bv{D}} + \bm{\Phi} \bv{Y}_t \sim \mathcal{N}\left(\overline{\bv{D}} + \bm{\Phi}\bm{\mu}_t , \bm{\Phi}\bm{\Sigma}_t \bm{\Phi}^T \right),
\end{equation}
where 
\begin{alignat*}{2}
\bm{\mu}_t&:=\overline{\bv{Y}}+ \left[\mu_t^1,\dots,\mu_t^R\right]^T\in\mathbb{R}^{R \times 1}, \\ \bm{\Sigma}_t&:=\textrm{diag}\left(\Sigma_t^1,\dots,\Sigma_t^{R}\right)\in\mathbb{R}^{R \times R}.\end{alignat*} 
Both $\mu_t^j\in\mathbb{R}$ and $\Sigma_t^j\in\mathbb{R}$ are evaluated for each of the $R$ GPs, using respectively \autoref{eq:gpposteriormean} and \autoref{eq:gpposteriorcovariance} with $Q=t$. The spatio-temporal distribution of uncertainties  $\bv{U}_t$ in the motion-fields can be obtained as the diagonal of the covariance matrix in \autoref{eq:gp_dvf_distribution}: $$[\bv{U}_t]_i = \sum_{j=1}^R \Sigma_t^j [\bm{\Phi}]_i^2. $$




\subsubsection{Fitting a GP to motion representation coefficients}
\label{section:theory_fittingp}
We assume that each (zero-mean) representation coefficient ${Y}_t^j\in\mathbb{R}$, for $j=1,\dots,N_p$, can be modeled as a function of the latent representation of three mutually orthogonal $k$-space spokes,  $\bv{X}_t=\bv{U}^\dagger \bv{S}_t \in \mathbb{C}^{3 N_X \times 1}$, where $\bv{S}_t$ denotes the original spokes. That is, we assume there exist functions $g^j \sim \mathcal{GP}(0,k^j)$ such that $$Y^j_t = g^j(\bv{X}_t) + {\epsilon}^j, $$ for Gaussian noise  ${\epsilon}^j \sim \mathcal{N}(0,\left(\sigma^j_n\right)^2 )$. Similar to \autoref{eq:drawfromgp}, note that this defines a Gaussian likelihood over $\mathcal{T}$
\begin{equation}
\label{eq:gptraininglikelihood}
\bv{Y}_\mathcal{D}^j \sim \mathcal{N}\left(\bv{0},\bm{\Sigma}_\mathcal{D}^j + \left(\sigma_n^j\right)^2 \bv{I} \right), \end{equation} 
with $\bm{\Sigma}^j_\mathcal{D}:=k^j(\bv{X}_\mathcal{D},\bv{X}_\mathcal{D} | \bm{\theta}^j_k )$. Next, a single-output GP is fit per representation coefficient ($R$ in total) to the corresponding pair-wise training data $\mathcal{T}^j=\{ \bv{X}_\mathcal{D}, \bv{Y}^j_\mathcal{D} \},$ consisting of the three mutually orthogonal, respiratory-sorted $k$-space readouts and the $j$-th respiratory-sorted motion-field representation coefficient. The fitting is done by maximizing the Gaussian likelihood \autoref{eq:gptraininglikelihood} through MLE with respect to the GP's hyperparameters $\bm{\theta}^j:=\{\bm{\theta}^j_k , \sigma^j_n \}$.  The result of this step is a prior distribution for each motion representation coefficient.









%==========================

\subsubsection{Online inference phase} 
\label{section:reconstructiondetails_onlineinference}



Now that all parameters in the pipeline in \autoref{eq:methodpipeline} are determined - GP hyperparameters, and dimension reduction bases - and a rejection criterion is defined, the complete pipeline can be evaluated in the online inference phase. Given a newly acquired set of three-mutually orthogonal spokes $\bv{X}_t$ at time $t$, the most-likely representation coefficients and prediction uncertainty are evaluated in the order of milliseconds as respectively the posterior mean and covariances from \autoref{eq:gpposteriormean} and \autoref{eq:gpposteriorcovariance}, and subsequently \autoref{eq:gp_dvf_distribution}, with $\bv{X}_Q:=\bv{X}_t$. 

The result of this step is the most likely 3D motion-field, the corresponding 3D spatial estimation uncertainty map, and a flag whether or not the motion model $\bm{\Phi}$ that is used in the pipeline is applicable for this newly acquired data. Both the data acquisition and the 3D motion-field inference could be performed at extremely high speeds of around 70 Hz with $TR=4.8\textrm{ ms}$. In practice, if a flag is raised, the uncertainty in the motion estimates is too high, and the radiation treatments should be stopped, and possibly continued whenever confidence is restored.



% \subsection{Gaussian Process for regression}
% \label{section:gppriordistribution}
% Formally, a Gaussian Process (GP) is defined as a collection of random variables, any finite collection of which have joint Gaussian distributions \citep{rasmussen2003gaussian}. A GP is completely characterized in terms of its mean function $m(x)$ and its covariance, or kernel, function $k(x,x')$. To specify a Gaussian Process prior with mean $m$ and kernel $k$ over a function $y$, we write 
% \begin{equation}
% \label{eq:gaussianprocessdefinition}
% y \sim \mathcal{GP}(m, k).
% \end{equation} 
% The functions $m$ and $k$ are typically taken chosen from families of functions, and parameterized by hyperparameters, respectively defined as $\bm{\theta}_m$ and $\bm{\theta}_k$, that further specify their form within those families of functions. Given a certain choice for the mean and kernel functions, and a certain setting of hyperparameters, a GP specifies what function properties such as smoothness, jumps or periodicity are most likely. The GP can be considered as an extension of the Gaussian distribution; drawing a function from a GP, and sampling this function at a finite number of sample locations $\bv{X}$ specifies a multi-variate Gaussian random vector $\bv{Y}$
% \begin{equation}
% \label{eq:drawfromgp}
% \bv{Y}:=g(\bv{X}) \sim \mathcal{N}(\bv{m}_\bv{X},\bv{K}_{\bv{X},\bv{X}}),
% \end{equation}
% with mean {\it vector} $\bv{m}_\bv{X}:=m(\bv{X} | \bm{\theta}_m)$ and covariance {\it matrix} $\bv{K}_{\bv{X},\bv{X}}:=k(\bv{X},\bv{X} | \bm{\theta}_k)$ defined as evaluations of the corresponding GP mean function $m$ and kernel function $k$. 

% In the rest of this work we can assume without loss of generality that $m \equiv 0$. Moreover, we assume pair-wise training data are available, $\mathcal{T}=\{\bv{X}_\mathcal{T},\bv{Y}_\mathcal{T}\}$, with sample locations $\bv{X}_\mathcal{T}$, and measurements $\bv{Y}_\mathcal{T}$. The GP can also be applied with noisy measurements $\bv{Y}_\mathcal{T}$ of the true underlying function $y \sim \mathcal{GP}(0,k)$. Similar to \autoref{eq:drawfromgp}, we then get 
% \begin{equation}
%     \label{eq:drawfromgp_noisy}
%     \bv{Y}_\mathcal{T} \sim \mathcal{N}(\bv{0},\bm{\Sigma}(\bm{\theta}_k)+\sigma_n^2 \bv{I})
% \end{equation} with Gaussian noise $\bm{\epsilon}\sim\mathcal{N}(\bv{0},\sigma_n^2\bv{I}).$ Note that this distribution over the training data is not yet fully specified; the hyperparameters $\bm{\theta}:=\{\bm{\theta}_k,\sigma_n\}$, including kernel hyperparameters and noise standard deviation, are still unknown. These can be optimized with maximum likelihood estimation (MLE) over the training data $\mathcal{T}$, yielding a fully-specified GP prior.

% \subsection{Gaussian Process - posterior distribution}
% In practice, Gaussian Processes can be used for regression, i.e. deducting true function values corresponding to (noisy) measurements, and predicting the most likely function values for unseen test cases. This requires to combine the GP prior from the previous section with measurements, which results in the GP posterior distribution. One of the major strengths of GPs, is that the GP posterior has a closed-form analytical expression that can be readily computed, which is in contrast with many other probabilistic frameworks that require approximation methods to estimate the posterior distribution.

% This closed-form expression for the posterior distribution over unseen function values $\bv{Y}_Q$ at newly queried test inputs $\bv{X}_Q$ can be derived from the assumption that $[\bv{Y}_\mathcal{T};\bv{Y}_Q]$ follows a joint Gaussian distribution with mean and covariance specified by the mean and kernel functions of the GP. Conditioning on the training data $\mathcal{T}$ then eventually yields  \citep{rasmussen2003gaussian}:
% \begin{equation}
% \label{eq:gpposterior_general}
% \bv{Y}_Q | \mathcal{T}  \sim \mathcal{N}\left(\bv{m}_Q , \bm{\Sigma}_Q \right),
% \end{equation}
% with 
% \begin{alignat}{2}
% \bv{m}_Q &= \bv{K}_{\mathcal{T},Q}^T\bv{K}_{\mathcal{T},\mathcal{T}}^{-1} \bv{Y}_\mathcal{T}, \label{eq:gpposteriormean}\\
% \bm{\Sigma}_Q &= \bv{K}_{QQ} - \bv{K}_{\mathcal{T},Q}^T \bv{K}_{\mathcal{T},\mathcal{T}}^{-1} \bv{K}_{\mathcal{T},Q}, \label{eq:gpposteriorcovariance}
% \end{alignat}
% Here we have defined the matrices $[\bv{K}_{A,B}]_{i,j}:=k(\bv{x}_i,\bv{x}_j)$, with $\bv{x}_i,\bv{x}_j$ defined as respectively the $i$-th and $j$-th columns in matrices $A$ and $B$. Evidently, the GP inference can be performed very efficiently, since it only involves evaluations of kernel matrices and matrix-vector products with the pre-computable matrix $\bv{K}_{\mathcal{T},\mathcal{T}}^{-1}$. In practice the inference can typically be done in the order of milliseconds.

%===================================
\subsection{Background on Gaussian Process Regression}
% \label{section:gpforregression}
%  The GP is completely characterized by its mean function $m(x)$ and kernel function $k(x,x)$, which in turn characterize a multi-variate Gaussian distribution:
% \begin{equation}
% \label{eq:drawfromgp}
% Y_\bv{x}|\bv{x} \sim \mathcal{N}(\bv{m}_\bv{x},\bv{K}_{\bv{x},\bv{x}}),
% \end{equation}
% where $\bv{m}_\bv{x}$ and $\bv{K}_{\bv{x},\bv{x}}$ denote evaluations of respectively the mean and kernel function for all samples in $\bv{x}$.
% Equivalently stated, a GP prior is placed over $y$, i.e.
% \begin{equation}
%     \label{eq:gpprior}
%     y \sim \mathcal{GP}(m,k).
% \end{equation}

A Gaussian Process (GP) \citep{rasmussen2003gaussian} models a Gaussian probability distribution over functions, and can therefore be considered as an extension of the multi-variate Gaussian distribution which models a Gaussian probability distribution over vectors. Gaussian Processes are frequently applied to regression problems by assuming the following model for noisy measurements $\bv{y}_t
\in\mathcal{Y}\subset\mathbb{R}^{N_\mathcal{Y} \times 1}$ at measurements $\bv{x}_t \in \mathcal{X} \subset \mathbb{C}^{N_\mathcal{X} \times 1}$: 
\begin{equation}\label{eq:noisymeasurementmodel} \bv{y}_t = \bm{y}(\bv{x}_t)+\bm{\epsilon},\end{equation}
where $\bm{\epsilon}\in\mathcal{X},\bm{\epsilon}\sim\mathcal{N}(\bv{0},\sigma_n^2 \bv{I}$), and $\bm{y}:\mathcal{X}\rightarrow\mathcal{Y}$. In a specific scenario, GPs define a multi-variate Gaussian distribution: in case a function is drawn from a GP, and evaluated at a finite collection of $N_\mathcal{T}$ measurements $\bv{x}_1,\dots,\bv{x}_{N_\mathcal{T}}$, then the corresponding function values $\bv{y}_\mathcal{T}:=[\bv{y}_1;\dots; \bv{y}_{N_\mathcal{T}}]$ follow a multi-variate Gaussian distribution. Similar to a mean vector and kernel matrix, a GP is completely characterized by a mean $m(x)$, and kernel {\it function} $k(x_i,x_j)$, which in turn specify the mean vector and kernel matrix of the corresponding multi-variate Gaussian distribution: \begin{equation}
\label{eq:drawfromgp}
\bv{y}_\mathcal{T}|\mathcal{T} \sim \mathcal{N}(\bv{m}_\mathcal{T},\bv{K}_{\mathcal{T},\mathcal{T}}),
\end{equation}
where $\mathcal{T}$ is defined as the training set $\mathcal{T}:=\{(\bv{x}_i,\bv{y}_i)\}_{i=1}^{N_\mathcal{T}}$, and $\bv{m}_\mathcal{T}$ and $\bv{K}_{\mathcal{T},\mathcal{T}}$ denote evaluations of respectively the mean and kernel function for all training samples in $\mathcal{T}$. The kernel function characterizes the properties (e.g. smoothness, periodicity, etc) of the functions that are modeled by the GP. For this reason, application of the GP model as described above is also typically referred to as placing a GP prior over $y$: \begin{equation}
    \label{eq:gpprior}
    y \sim \mathcal{GP}(m,k).
\end{equation}
Without loss of generality, it is typically assumed that $m \equiv 0$, in which case the GP prior is completely characterized by the kernel function. Intuitively, the GP prior assumes that if two measurements are considered similar by the kernel function, then the corresponding function values will be similar as well. A kernel function is chosen from families of functions based on some prior knowledge on $y$ (e.g. periodicity, or smoothness in time), and parameterized by hyperparameters $\bm{\theta}$ that determine its final form. 



Evidently, correct tuning of these $\bm{\theta}$ in the GP prior directly influences the GP's regression performance. Therefore, two steps are followed to perform GP-based regression. In the first step the GP prior is optimized: the GP hyperparameters are estimated given a pair-wise training set $\mathcal{T}=\{ (\bv{x}_{t},\bv{y}_{t})\}_{t\in\mathcal{T}}$ with observed function values $\bv{y}_t$ and measurement locations $\bv{x}_t$, the probability of making these observations is maximized by maximum likelihood estimation (MLE) on the joint Gaussian likelihood \eqref{eq:drawfromgp}. The result is a fully-specified GP prior, specifying the properties of the functions that best fit the training measurements. However, for regression, not only the function properties, but also the actually measured function values need to be taken into account. This is done in the second step as follows. The GP prior defines a joint prior distribution over any set of measurements, including the set of observed noisy measurements $\bv{y}_\mathcal{T}$ concatenated with the unknown noise-free function values $\bv{y}_Q$ at queried measurement locations $\bv{x}_Q$:
\begin{equation}
\label{eq:drawfromjointgp}
\begin{bmatrix} \bv{y}_\mathcal{T} \\ \bv{y}_Q  \end{bmatrix} \sim \mathcal{N}\left(\bv{0},\begin{bmatrix} \bv{K}_{\mathcal{T},\mathcal{T}} + \sigma_n^2 \bv{I} & \bv{K}_{\mathcal{T},\mathcal{Q}} \\ \bv{K}_{\mathcal{T},\mathcal{Q}}^T & \bv{K}_{Q,Q}  \end{bmatrix} \right)
\end{equation}
Here we have defined the matrices $[\bv{K}_{A,B}]_{i,j}:=k(\bv{x}_i,\bv{x}_j)$, with $\bv{x}_i,\bv{x}_j$ defined as respectively the $i$-th and $j$-th columns in matrices $A$ and $B$. Note the occurrence of the standard deviation $\sigma_n$, of the target noise $\bm{\epsilon}$ in \autoref{eq:noisymeasurementmodel}. In the second step, a distribution over the unseen function values is evaluated by conditioning on the training data $\mathcal{T}$, yielding the Gaussian posterior distribution (\citet{rasmussen2003gaussian}, Eq. [A.6] ):
\begin{equation}
\label{eq:gpposterior_general}
\bv{y}_Q | \mathcal{T}  \sim \mathcal{N}\left(\bv{m}_Q , \bm{\Sigma}_Q \right),
\end{equation}
with 
\begin{alignat}{2}
\bv{m}_Q &= \bv{K}_{\mathcal{T},Q}^T\left(\bv{K}_{\mathcal{T},\mathcal{T}}+\sigma_n^2 \bv{I}\right)^{-1} \bv{y}_\mathcal{T}, \label{eq:gpposteriormean}\\
\bm{\Sigma}_Q &= \bv{K}_{QQ} - \bv{K}_{\mathcal{T},Q}^T \left(\bv{K}_{\mathcal{T},\mathcal{T}}+\sigma_n^2 \bv{I}\right)^{-1} \bv{K}_{\mathcal{T},Q}. \label{eq:gpposteriorcovariance}
\end{alignat}
The diagonal elements of $\bm{\Sigma}_Q$ define the GP prediction uncertainty. 

Since the GP performs regression on the function $\bm{y}:\mathcal{X}\rightarrow\mathcal{Y}$, the posterior can be interpreted as an approximation of this function, mapping measurements in $\mathcal{X}$ to the most-likely function values and uncertainties in $\mathcal{Y}$:
\begin{equation}\mathcal{X} \xrightarrow[]{\hspace{.4cm}\textrm{GP}\hspace{.4cm}} \mathcal{Y}. \end{equation}
%=======================================

%overview again??


Next, the motion model is applied to expand the GP outputs $\bv{y}_t$, yielding 3D motion-fields $\bm{\Phi}\bv{y}_t=\bv{d}_t \subset \mathcal{D}$. Altogether the pipeline is executed by projection acquired spokes $\bv{s}_t$ onto $\mathcal{X}$ as $\bv{x}_t=\bv{U}^\dagger \bv{s}_t$, which are then input to the GP resulting in the distribution $P(\bv{y}_t | \bv{s}_t )$, to which the motion model is applied. Due to the linear nature of the whole pipeline, the result is a posterior distribution over motion-fields conditioned on the input spokes, i.e. $P(\bv{d}_t =\bm{\Phi}\bv{y}_t |\bv{s}_t)$. Finally, a real-time quality assurance criterion based on the posterior uncertainty is evaluated, thereby flagging dynamics with potentially erroneous motion estimates.
%==========================================

==> sections/figures.tex <==

%% =========== New figures BELOW ===========



\clearpage
\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{overview_figure.pdf}
    \caption{Framework overview. In the training phase, GM3DR+SN data is acquired during 3 minutes of free-breathing. The motion model and spoke compression basis are built with PCA on respectively respiratory-sorted GM3DR+SN and SN spokes. The motion model requires motion-fields, which are obtained by Optical Flow \citep{zachiu2015improved} on respiratory-sorted images. Finally, GP hyperparameters $\bm{\theta}$ are obtained by maximum likelihood estimation on the training set $\mathcal{T}=\{(\bv{x}_i,\bv{y}_i)\}_{i=1}^M$, consisting of the compressed spoke representations $\bv{x}_i$ and motion-fields representation coefficients $\bv{y}_i$. In the inference phase three steps are followed: 1) SN spokes are compressed to $\bv{x}_t = \bv{U}^H \bv{s}_t$; 2) the posterior distribution $P(\bv{y}_t|\mathcal{T})$ is computed with the GP from $\bv{x}_t$; 3) a 3D motion-field $\bv{d}_t$ and a corresponding uncertainty map are inferred by expanding the GP posterior distribution with the motion model $\bm{\Phi}$.}
    \label{fig:frameworkoverview}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=.85\textwidth,height=0.28\textheight]{epe_boxplot_correlation.pdf}
    \caption{Left: correlation between end-point-error (EPE) and GP posterior uncertainty for all simulated breathing patterns. Note the log-scale on the $x$-axis. Additional analyses indicated for abdominal-only, chest-only and amplitude drifts, a correlation coefficient of respectively $\rho=0.99 \pm 0.00$, $\rho=0.99 \pm 0.00$ and $\rho=0.90 \pm 0.02$ $0.90 \pm 0.01$. Right: evaluation of the rejection criterion for all simulated breathing patterns; EPEs are computed before and after applying the rejection criterion. The notched boxplots indicate statistically significant ($p=0.05$) lower EPE before rejection than after rejection, showing the effectiveness to reject erroneous motion estimates.}
    \label{fig:correlation_epe_boxplots}
\end{figure*}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[trim={4.9cm 5.6cm 4.9cm 5cm},width=.5\textwidth]{correlation_uncertainty_epe_abdominalonlychestonlyamplitudedrifts.pdf}
%     \caption{For normal breathing -> abdominal-only. We could swap this with some statistical values (corr. coefficient + p-value). \url{https://towardsdatascience.com/eveything-you-need-to-know-about-interpreting-correlations-2c485841c0b8}}
%     \label{fig:correlation_epe_uncertainty}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[trim={5cm 5cm 5cm 5cm},width=.5\textwidth]{epe_boxplots_rejection_abdominalonlychestonlyamplitudedrifts.pdf}
%     \caption{Caption}
%     \label{fig:insilico_epe_boxplots}
% \end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{invivo_train_inf_zoom_allvols.pdf}
    \caption{Qualitative results of GP motion and uncertainty estimations in a digital phantom and five volunteers. The blue dots represent the training targets, the red line the posterior mean as estimated by the first GP - which corresponds to the first principal component of the motion model - from three readouts, and the gray shaded areas are the 95\% confidence intervals obtained from the estimation uncertainty as output by the GP. The first and second columns show an overview of respectively the training and the inference phase, the third column shows a zoom-in on a region with a slightly different motion pattern or increased estimation uncertainty. The increased uncertainty mostly occurs at the highest motion amplitude levels. Note that the units on the vertical axes are arbitrary; the scaling dependents on the magnitudes of the principal components in the motion model. However, in all cases the higher values indicate exhales, while the lower values indicate inhales.}
    \label{fig:robustnesstest_allvols}
\end{figure*}

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\textwidth]{invivo_inference_projections.pdf}
    \caption{Comparison between GP predictions and projection images. The image shows the comparison for all five volunteers between the posterior mean as estimated by the first GP corresponding to the first principal component of the motion model (green), projections on the FH-axis as obtained by an FFT over the readout of FH spokes (background), and rejected dynamics (red marks). The inference was performed on data acquired about two minutes after the training data were acquired.}
    \label{fig:robustness_projections_gm3dr}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{invivo_highspeed_inference_projections.pdf}
    \caption{High-speed in-vivo inference and quality assurance. The posterior mean of the first GP (green), and rejection criterion evaluations (red), are compared with projections on the FH-axis for all four volunteers with SN-only data available (2-5). Volunteers 3 and 5 were instructed to perform motion which would render the motion model invalid. Volunteer 3 performed in sequence: 1) normal breathing; 2) a switch to chest-only breathing; 3) bulk motion; 4) normal breathing, and the first abnormal event started around 535 seconds in the acquisition, as indicated by the yellow arrow. Volunteer 5 performed in sequence: 1) normal breathing; 2) irregular breathing; 3) bulk motion, and the first abnormal event started around 718 seconds in the acquisition, as indicated by the yellow arrow. The GP posterior means are scaled to visually overlap the pattern in the projection images.}
    \label{fig:highspeed_inference_allvols}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{drift_analysis.pdf}
    \caption{Analysis of the GP posterior uncertainties over the course of the whole acquisition. For volunteers 2-5 the acquisition switched to an SN-only acquisition at the end of the acquisition, indicated by the solid red line. A moving average filter with a window of 10 seconds is applied to the uncertainties to highlight the patterns over the whole acquisition rather than within the breathing cycles.}
    \label{fig:drift_analysis_allvols}
\end{figure*}
% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{invivo_highspeed_train_inf_zoom_vol3,5.pdf}
%     \caption{\colorred{ADD CAPTION, change axis, add zoom boxes, change breathing variation title}}
%     \label{fig:highspeed_inference_vol3,5}
% \end{figure*}


\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\textwidth]{rejection_val_com.pdf}
    \caption{This figure shows the result of the high-speed inference for volunteers 3 (left) and 5 (right), as discussed in \autoref{section:highspeedfeasibility_experiments} and \autoref{section:highspeedfeasibility_results}. The bottom graphs show a comparison with center-of-mass (COM) coordinates in left-right (orange) and feet-head (purple). The black arrows, labeled 1-4, indicate four events where the motion was changed, as can also be observed from the changing patterns in the COM-coordinates; 1) volunteer 3 switches breathing pattern, 2) volunteer 3 performs bulk motion, 3) volunteer 3 returns to normal breathing, 4) volunteer 5 performs bulk motion.}
    \label{fig:robustness_projections_sn}
\end{figure*}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth,height=0.4\textwidth]{invivo_flagging.pdf}
%     \caption{Qualitative evaluation of the rejection criterion on in vivo data. The model is trained on the first three minutes GM3DR data, and evaluated on all other data. For volunteer 1 the inference was performed on GM3DR data at 6.7 Hz, for all other volunteers it was performed on SN data at 69 Hz. }
%     \label{fig:robustness_projections_rejections}
% \end{figure*}




%% =========== New figures ABOVE ===========
%% =========== New figures ABOVE ===========
%% =========== New figures ABOVE ===========


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.3\textwidth]{epe_test_rejection_abdominalonly.png}
%     \caption{For normal breathing -> abdominal-only}
%     \label{fig:epe_rejection_test}
% \end{figure}






% \begin{figure*}[tbp]
% \centering
% \includegraphics[width=\textwidth]{invivo_boxplots.pdf}
% \caption{Boxplots of the posterior means (left) and posterior uncertainties (right) evaluated on two different sets of 30 consecutive seconds of free-breathing. Only the relative scale is important. The label 'GM3DR | SN' denotes a comparison between inference on the last 30 seconds of GM3DR data and the consecutive 30 seconds of SN spokes, the label 'GM3DR | GM3DR' denotes a comparison between inference on 30 seconds of the GM3DR data, and the consecutive 30 seconds of GM3DR data.}
% \end{figure*}

% vol 1
% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.7\textwidth]{flagged_dynamics_v1.png}
%     \caption{For volunteer 1: A golden-mean 3D radial (GM3DR) acquisition interleaved with FH, AP, LR self-navigation (SN) spokes. The model is trained on the first three minutes, tested on the rest, and the rejection criterion is determined on the last 30 seconds of training data. }
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.3\textwidth]{training_vs_testing_posterior_v1.png}
%     \caption{For volunteer 1: Boxplots of the posterior mean (left) and posterior uncertainty (right) evaluated on the last 30 seconds of the GM3DR+SN data (green), and the first 30 seconds of the SN data (orange). Only the relative scale is important. A relatively steady breathing pattern seems evident from the posterior mean, but the posterior uncertainty is slightly larger in the inference phase.}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}



% vol 2
% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.7\textwidth]{flagged_dynamics_v2.png}
%     \caption{For volunteer 2: A golden-mean 3D radial (GM3DR) acquisition interleaved with FH, AP, LR self-navigation (SN) spokes. The model is trained on the first three minutes of GM3DR+SN, tested on the rest, and the rejection criterion is determined on the last 30 seconds of training data. After the GM3DR+SN acquisition, only the SN spokes are acquired at around 70 Hz. The model is evaluated on both the GM3DR+SN and SN data. Note the change in resolution due to the switch in trajectory.}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.3\textwidth]{training_vs_testing_posterior_v2.png}
%     \caption{For volunteer 2: Boxplots of the posterior mean (left) and posterior uncertainty (right) evaluated on the last 30 seconds of the GM3DR+SN data (green), and the first 30 seconds of the SN data (orange). Only the relative scale is important. A relatively steady breathing pattern seems evident from the posterior mean, but a large difference remains for the uncertainty during training and during testing.}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}


% vol 3
% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.7\textwidth]{flagged_dynamics_v3.png}
%     \caption{For volunteer 3: A golden-mean 3D radial (GM3DR) acquisition interleaved with FH, AP, LR self-navigation (SN) spokes. The model is trained on the first three minutes of GM3DR+SN, tested on the rest, and the rejection criterion is determined on the last 30 seconds of training data. After the GM3DR+SN acquisition, only the SN spokes are acquired at around 70 Hz. The model is evaluated on both the GM3DR+SN and SN data. Note the change in resolution due to the switch in trajectory. This volunteer was asked to first switch to chest breathing (starts around halfway), then switch back to normal breathing and perform bulk motion (starts around 3/4).}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.3\textwidth]{training_vs_testing_posterior_v3.png}
%     \caption{For volunteer 3: Boxplots of the posterior mean (left) and posterior uncertainty (right) evaluated on the last 30 seconds of the GM3DR+SN data (green), and the first 30 seconds of the SN data (orange). Only the relative scale is important. A relatively steady breathing pattern seems evident from the posterior mean, but a difference remains between the uncertainty during training and during testing. }
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}

% vol 4
% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.7\textwidth]{flagged_dynamics_v4.png}
%     \caption{For volunteer 4: A golden-mean 3D radial (GM3DR) acquisition interleaved with FH, AP, LR self-navigation (SN) spokes. The model is trained on the first three minutes of GM3DR+SN, tested on the rest, and the rejection criterion is determined on the last 30 seconds of training data. After the GM3DR+SN acquisition, only the SN spokes are acquired at around 70 Hz. The model is evaluated on both the GM3DR+SN and SN data. Note the change in resolution due to the switch in trajectory. For this volunteer the GM3DR+SN phase in the beginning is longer since no breath-hold was performed in the complete acquisition, resulting in more free-breathing GM3DR+SN data.}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}

% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=0.3\textwidth]{training_vs_testing_posterior_v4.png}
%     \caption{For volunteer 4: Boxplots of the posterior mean (left) and posterior uncertainty (right) evaluated on the last 30 seconds of the GM3DR+SN data (green), and the first 30 seconds of the SN data (orange). Only the relative scale is important. A small drift in the superior direction seems evident from the posterior mean, but a large difference remains between the uncertainty during training and during testing.}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure}

% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=0.3\textwidth]{training_vs_gm3dr_testing_posterior_v4.png}
%     \caption{For volunteer 4: Boxplots of the posterior mean (left) and posterior uncertainty (right) evaluated on first 30 seconds of the GM3DR+SN data (green), and the last 30 seconds of the GM3DR+SN data (orange). Only the relative scale is important. Note the difference with the previous figure: the breathing pattern appear steady, and the posterior uncertainty is similar. This indicates that the SN-data could have more artefacts than GM3DR+SN data, which directly influences the posterior uncertainty.}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure}

% vol 5
% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.7\textwidth]{flagged_dynamics_v5.png}
%     \caption{For volunteer 5: A golden-mean 3D radial (GM3DR) acquisition interleaved with FH, AP, LR self-navigation (SN) spokes. The model is trained on the first three minutes of GM3DR+SN, tested on the rest, and the rejection criterion is determined on the last 30 seconds of training data. After the GM3DR+SN acquisition, only the SN spokes are acquired at around 70 Hz. The model is evaluated on both the GM3DR+SN and SN data. Note the change in resolution due to the switch in trajectory. This volunteer was asked to perform bulk motion (end of the scan).}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.3\textwidth]{training_vs_testing_posterior_v5.png}
%     \caption{For volunteer 5: Boxplots of the posterior mean (left) and posterior uncertainty (right) evaluated on the last 30 seconds of the GM3DR+SN data (green), and the first 30 seconds of the SN data (orange). Only the relative scale is important. A relatively large drift in the superior direction seems evident from the posterior mean, and a large difference remains between the uncertainty during training and during testing.}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}



% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=0.7\textwidth]{gp_bulkmotion_detection_invivo.png}
%     \caption{For volunteer 1}
%     \label{fig:gp_bulkmotion_detection_invivo}
% \end{figure*}


==> sections/supporting_figures.tex <==
\graphicspath{{./figures/}}

\clearpage
\setsuppfig
\setcounter{figure}{0}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{invivo_averaging_vol3.pdf}
    \caption{The effect of temporally averaging the input SN-spokes. Several reconstructions of the first GP for volunteer 3 are shown for which a symmetric moving mean filter is applied with a varying width: 1, 27, 40, 60, 80, and 200 dynamics. This averaging increases the temporal latency, as indicated in the titles, since the data required by the second half of the window lies in the future. However, evidently, the filtering also results in smoother reconstructions. Hence, temporal filtering allows to make a trade-off between the temporal resolution of the reconstructions and the SNR. Temporal averaging with a width of 27 dynamics would result in sufficient temporal resolution for real-time adaptive MRgRT \citep{Murphy2002,keall2006management}.}
    \label{supfig:averaging_vol3}
\end{figure*}
